Revisiting Tri-training of Dependency Parsers

We compare two orthogonal semi-supervised learning techniques, namely tri-training and pretrained word embeddings, in the task of dependency parsing. We explore language-specific FastText and ELMo embeddings and multilingual BERT embeddings. We focus on a low resource scenario as semi-supervised learning can be expected to have the most impact here. Based on treebank size and available ELMo models, we select Hungarian, Uyghur (a zero-shot language for mBERT) and Vietnamese. Furthermore, we include English in a simulated low-resource setting. We find that pretrained word embeddings make more effective use of unlabelled data than tri-training but that the two approaches can be successfully combined.

==> 90x-appendices/0633-aug-table-vertical.tex <==
\begin{table}
\centering
\begin{tabular}{l|l|r|r|r}
\multicolumn{5}{l}{\textit{(i)} Small $A$}\\
\textbf{Lang.} & \textbf{Parser} & \textbf{5k} & \textbf{10k} & \textbf{20k}\\
\hline
\multirow{2}{*}{e} & f & 77.5 & 77.9 & \textbf{78.2} \\
 & h & 84.1 & 84.4 & \textbf{84.6} \\
\hline
\multirow{2}{*}{h} & f & 80.2 & 81.1 & \textbf{81.1} \\
 & h & 85.3 & 85.7 & \textbf{85.7} \\
\hline
\multirow{2}{*}{u} & f & 67.5 & 67.9 & \textbf{68.5} \\
 & h & 71.6 & 71.7 & \textbf{71.7} \\
\hline
\multirow{2}{*}{v} & f & 63.6 & 63.7 & \textbf{64.2} \\
 & h & \textbf{67.8} & 67.7 & 67.7 \\
\hline
\\
\multicolumn{5}{l}{\textit{(ii)} Medium $A$}\\
\textbf{Lang.} & \textbf{Parser} & \textbf{20k} & \textbf{40k} & \textbf{80k}\\
\hline
\multirow{2}{*}{En} & f & 77.4 &         77.8  & \textbf{78.3} \\
                   & h & 84.2 &         84.4  & \textbf{84.5} \\
\hline
\multirow{2}{*}{Hu} & f & 80.3 &         80.7  & \textbf{81.1} \\
                   & h & 85.3 &         85.4  & \textbf{85.7} \\
\hline
\multirow{2}{*}{Ug} & f & 67.6 &         67.9  & \textbf{68.4} \\
                   & h & 71.4 &         71.5  & \textbf{71.7} \\
\hline
\multirow{2}{*}{Vi} & f & 63.4 &         63.8  & \textbf{64.2} \\
                   & h & 67.5 & \textbf{67.6} &         67.6 \\
\hline
\\
\multicolumn{5}{l}{\textit{(iii)} Big $A$} \\
\textbf{Lang.} & \textbf{Parser} & \textbf{80k} & \textbf{160k} & \textbf{$\Delta$}\\
\hline
\multirow{2}{*}{e} & f & 78.0 & \textbf{78.4} & 0.4 \\
 & h & 84.2 & \textbf{84.4} & 0.2 \\
\hline
\multirow{2}{*}{h} & f & 80.8 & \textbf{81.3} & 0.5 \\
 & h & 85.6 & \textbf{85.8} & 0.3 \\
\hline
\multirow{2}{*}{u} & f & 68.2 & \textbf{68.4} & 0.2 \\
 & h & 71.7 & \textbf{71.9} & 0.1 \\
\hline
\multirow{2}{*}{v} & f & 63.9 & \textbf{64.0} & 0.1 \\
 & h & 67.6 & \textbf{68.0} & 0.5 \\
\hline
\end{tabular}
\caption{Effect of augmentation size $A$ on tri-training
    performance (average development LAS over multiple tri-training runs, selecting, for each run, the best tri-training iteration according to development LAS):
    \textit{(i)} two runs
        for each setting (language, parser, augmentation size)
        with $T=16$, seed data sampled as 250\% of labelled data,
        $d=1$ 
        ,
    \textit{(ii)} three runs (Uygur) or four runs (other languages)
        for each setting (language, parser, augmentation size)
        with $T=8$, seed data sampled as 250\% of labelled data,
        $d=1$ 
        ,
    \textit{(iii)} six runs
        for each setting (language, parser, augmentation size)
        with $T=4$, seed data sampled as 100\% or 250\% of labelled data,
        $d=0.5$ 
        .
    }
\label{tab:augsize-effect}
\end{table}
